BOTTER: A framework to analyze social bots in Twitter

Social networks have triumphed in communicating people online, but they have also been exploited to launch influence operations for manipulating society. The deployment of software-controlled accounts (e.g., social bots) has proven to be one of the most effective enablers for that purpose, and tools for their detection have been developed and widely adopted. However, the way to analyze these accounts and measure their impact is heterogeneous in the literature, where each case study performs unique measurements. To unify these efforts, we propose a common framework to analyze the interference of social bots in Twitter. The methodology compares the non-authentic actors with the rest of users from different perspectives, thus building objective metrics to measure their actual impact. We validate the framework by applying it to a dataset of Twitter iterations dated in the weeks preceding the 2019 Spanish general election. In this sense, we check that our framework facilitates the quantitative evaluation of unauthentic groups, particularly discovering that social bots changed the natural dynamics of the network in these days, but did not have a significant impact. We also consider this methodology as a practical tool for the qualitative interpretation of experimental results, particularly suggesting within the aforementioned electoral context that semi-automated accounts are potentially more threatening than fully automated ones.

==> framework.tex <==
\section{Framework design properties}\label{framework-design}
This framework defines a guided methodology to measure the interference of certain users (\eg social bots, fake news spreaders, or a specific subset of accounts) on social network dynamics in relation with the rest of actors. This comparative perspective exposes malicious patterns and corrupted properties which suggest whether or not the targeted groups have actually impacted and influenced on the system. The framework has been designed to fulfil the following properties:

\begin{itemize}
    \item \textbf{Comparative}: The methodology begins with the definition of groups (usually \textit{humans} and \textit{bots}), which are subsequently evaluated from different perspectives.
    
    \item \textbf{Computational}: Data is the vertebral axis of the model, enabling the application of statistical theories, data mining techniques, and artificial intelligence algorithms.
    
    %\item \textbf{Network-based}: Users and their relationships are represented in social graphs, widely adopted for representing social network dynamic \cite{barabasi2013network}.
    
    \item \textbf{Objective}: From the aforementioned points, the proposed methodology is based on proven and well-known algorithms, metrics, and properties, which do not permit biased diagnostics or subjective interpretations.
    
    \item \textbf{Generalizable}: Although the initial motivation of this framework is about determining the impact of social bots, the methodology is suitable for analyzing any kind of group of users (\textit{influencers}, verified accounts, or with any other condition).
    
    \item \textbf{Decoupled}: Methodology perspectives can be adopted independently without the need to implement the overall workflow. This flexibility is valuable for analysts interested in exploring specific particularities of the targeted group.
    
    \item \textbf{Extensible}: The proposal is the first approach towards the standardization of impact measurement of particular groups of users on social circles. Therefore, it constitutes a basic but solid baseline supported by widely proven metrics from which to incorporate improvements and build new perspectives.
\end{itemize}

Section~\ref{sec:framework-phases} describes in detail the phases that compose the methodology.













